Palette-based image decomposition, harmonization, and color transfer

We present a palette-based framework for color composition for visual applications. Color composition is a critical aspect of visual applications in art, design, and visualization. The color wheel is often used to explain pleasing color combinations in geometric terms, and, in digital design, to provide a user interface to visualize and manipulate colors. We abstract relationships between palette colors as a compact set of axes describing harmonic templates over perceptually uniform color wheels. Our framework provides a basis for a variety of color-aware image operations, such as color harmonization and color transfer, and can be applied to videos. To enable our approach, we introduce an extremely scalable and efficient yet simple palette-based image decomposition algorithm. Our approach is based on the geometry of images in RGBXY-space. This new geometric approach is orders of magnitude more efficient than previous work and requires no numerical optimization. We demonstrate a real-time layer decomposition tool. After preprocessing, our algorithm can decompose 6 MP images into layers in 20 milliseconds. We also conducted three large-scale, wide-ranging perceptual studies on the perception of harmonic colors and harmonization algorithms.

==> star_tessellation.tex <==
\begin{algorithm}
\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
\KwIn{Palette $\mathbf{P}$ with shape $M*3$; Color points $\mathbf{I}$, with shape $N*3$. $N$ is color points number, $M$ is palette size.}
\KwOut{Mixing weights $\mathbf{W}$, with shape $N*M$}
star $\gets$ ClosestToBlackPoint($\mathbf{P}$) \;
hullFaces $\gets$ ConvexHull($\mathbf{P}$) \;
$i \gets 0$ \; 
$Q \gets len(hullFaces)$\;
$\mathbf{W} \gets$ \o \;
\While{ $i<Q$}
{
    face $\gets$ hullFaces($i$) \;
    \If {star $\not\in$ face}
    {
     //Make a tetrahedron by linking star point with surface triangle. \;
     tetrahedron $\gets$ star $\cup$ face \;\;

     //Find color points that are inside this tetrahedron. \;
     $\mathbf{I}_{\{i\}} \gets$ InsideTetrahedronPointSet(tetrahedron, $\mathbf{I}$) \;\;

     //Call function defined in Figure~\ref{fig:decomposition_algorithm} to get barycentric coordinates for these inside color points. \

     $\mathbf{B}_{\{i\}} \gets$  Delaunay\_coordinates(tetrahedron, $\mathbf{I}_{\{i\}}$) \;\;

     // Mapping from barycentric to Whole Palette mixing weights. \;
     $\mathbf{W}_{\{i\}} \gets$ MappingFromTetrachdronToPalette($\mathbf{B}_{\{i\}}$) \;\;
     
     //Merge mixing weights $\mathbf{W}_{\{i\}}$ of color points set $\mathbf{I}_{\{i\}}$ into total mixing weights according to color points index. \;
     $\mathbf{W} \gets \mathbf{W} \cup \mathbf{W}_{\{i\}}$ \;
    }
    $i \gets i+1$ \;
}
\Return{$\mathbf{W}$}\;
\caption{Our Star triangulation barycentric coordinates algorithm.}
\label{algo:star_triangulation}
\end{algorithm}

